Landscapes at Colliders

Theories with a large number of long-lived metastable vacua are our only concrete explanation for the puzzling value of the Cosmological Constant (CC). The energy scales where these vacua are realized are unknown. In this work, we consider the possibility that a sector of this landscape of vacua is within experimental reach and discuss its signatures at colliders. We find that striking large-multiplicity final states might have gone undetected due to their relatively small total energy. In particular, this could lead to new exotic Higgs decays, which are both intriguing and challenging to search for. In addition to a general phenomenological analysis of these theories, we also discuss an explicit model where the small values of the CC and the Higgs mass are jointly explained by Weinberg's anthropic argument and a low energy landscape.

==> header.tex <==
% *****************************************************************
% ********************** BEGIN HEADER **********************
% *****************************************************************

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%PACKAGES
\usepackage{amsmath}	% AMS Math Package
\usepackage{amsthm}		% Theorem Formatting
\usepackage{amssymb}	% Math symbols such as \mathbb
\usepackage{eufrak}
\usepackage{datetime}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{verbatim}
\usepackage{bm}
\usepackage{float}
%\usepackage{tabularx}

\usepackage[colorlinks=true, citecolor=midblue, linkcolor=midblue, urlcolor=midblue]{hyperref}

\usepackage{setspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%COLOURS
%existing: black, white, blue, red, green, yellow
\definecolor{grey}{rgb}{0.4,0.4,0.4}
\definecolor{dullmagenta}{rgb}{0.4,0,0.4}
\definecolor{darkblue}{rgb}{0,0,0.4}
\definecolor{midblue}{rgb}{0,0,0.5}
\definecolor{midred}{rgb}{0.5,0,0}
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{lightbrown}{rgb}{0.75,0.5,0.25}
\definecolor{tan}{cmyk}{0.14,0.42,0.56,0}
\definecolor{djunglegreen}{cmyk}{0.99,0,0.52,0}
\definecolor{lightgreen}{rgb}{0,1,0}
\definecolor{olivegreen}{cmyk}{0.64,0,0.95,0.40}
\definecolor{midgreen}{rgb}{0.0,0.675,0.0}
\definecolor{darkgreen}{rgb}{0,0.5,0}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%NORMS
\newcommand{\normsingle}[1]{\left|{#1}\right|}
\newcommand{\normdouble}[1]{\left\|{#1}\right\|}
%\newcommand{\normtriple}[1]{\left\interleave{#1}\right\interleave} % requires ``stmaryrd'' package
\newcommand{\norm}[1]{\normdouble{#1}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%SHIFTS
\newcommand{\q}{\quad}
\newcommand{\qq}{\qquad}
\newcommand{\qqq}{\qquad\quad}
\newcommand{\qqqq}{\qquad\qquad}
\newcommand{\vs}{\vspace}
\newcommand{\hs}{\hspace}
\renewcommand{\.}{\hspace{0.5mm}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%ARROWS
\newcommand{\ra}{\ensuremath{\rightarrow}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\Ra}{\ensuremath{\Rightarrow}}
\newcommand{\La}{\ensuremath{\Leftarrow}}
\newcommand{\lra}{\ensuremath{\leftrightarrow}}
\newcommand{\Lra}{\ensuremath{\Leftrightarrow}}
\newcommand{\Ral}{\ensuremath{\Longrightarrow}}
\newcommand{\Lal}{\ensuremath{\Longleftarrow}}
\newcommand{\Lral}{\ensuremath{\Longleftrightarrow}}
\newcommand{\lral}{\ensuremath{\ongleftrightarrow}}
\newcommand{\ral}{\ensuremath{\longrightarrow}}
\newcommand{\lal}{\ensuremath{\longleftarrow}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%MATHEMATICS

%%%capital \mathrm
\newcommand{\Arm}{\ensuremath{\mathrm{A}}}
\newcommand{\Brm}{\ensuremath{\mathrm{B}}}
\newcommand{\Crm}{\ensuremath{\mathrm{C}}}
\newcommand{\Drm}{\ensuremath{\mathrm{D}}}
\newcommand{\Erm}{\ensuremath{\mathrm{E}}}
\newcommand{\Frm}{\ensuremath{\mathrm{F}}}
\newcommand{\Grm}{\ensuremath{\mathrm{G}}}
\newcommand{\Hrm}{\ensuremath{\mathrm{H}}}
\newcommand{\Irm}{\ensuremath{\mathrm{I}}}
\newcommand{\Jrm}{\ensuremath{\mathrm{J}}}
\newcommand{\Krm}{\ensuremath{\mathrm{K}}}
\newcommand{\Lrm}{\ensuremath{\mathrm{L}}}
\newcommand{\Mrm}{\ensuremath{\mathrm{M}}}
\newcommand{\Nrm}{\ensuremath{\mathrm{N}}}
\newcommand{\Orm}{\ensuremath{\mathrm{O}}}
\newcommand{\Prm}{\ensuremath{\mathrm{P}}}
\newcommand{\Qrm}{\ensuremath{\mathrm{Q}}}
\newcommand{\Rrm}{\ensuremath{\mathrm{R}}}
\newcommand{\Srm}{\ensuremath{\mathrm{S}}}
\newcommand{\Trm}{\ensuremath{\mathrm{T}}}
\newcommand{\Urm}{\ensuremath{\mathrm{U}}}
\newcommand{\Vrm}{\ensuremath{\mathrm{V}}}
\newcommand{\Wrm}{\ensuremath{\mathrm{W}}}
\newcommand{\Xrm}{\ensuremath{\mathrm{X}}}
\newcommand{\Yrm}{\ensuremath{\mathrm{Y}}}
\newcommand{\Zrm}{\ensuremath{\mathrm{Z}}}
%%%small \mathrm
\newcommand{\arm}{\ensuremath{\mathrm{a}}}
\newcommand{\brm}{\ensuremath{\mathrm{b}}}
\newcommand{\crm}{\ensuremath{\mathrm{c}}}
\newcommand{\drm}{\ensuremath{\mathrm{d}}}
\newcommand{\erm}{\ensuremath{\mathrm{e}}}
\newcommand{\frm}{\ensuremath{\mathrm{f}}}
\newcommand{\grm}{\ensuremath{\mathrm{g}}}
\newcommand{\hrm}{\ensuremath{\mathrm{h}}}
\newcommand{\irm}{\ensuremath{\mathrm{i}}}
\newcommand{\jrm}{\ensuremath{\mathrm{j}}}
\newcommand{\krm}{\ensuremath{\mathrm{k}}}
\newcommand{\lrm}{\ensuremath{\mathrm{l}}}
\newcommand{\mrm}{\ensuremath{\mathrm{m}}}
\newcommand{\nrm}{\ensuremath{\mathrm{n}}}
\newcommand{\orm}{\ensuremath{\mathrm{o}}}
\newcommand{\prm}{\ensuremath{\mathrm{p}}}
\newcommand{\qrm}{\ensuremath{\mathrm{q}}}
\newcommand{\rrm}{\ensuremath{\mathrm{r}}}
\newcommand{\srm}{\ensuremath{\mathrm{s}}}
\newcommand{\trm}{\ensuremath{\mathrm{t}}}
\newcommand{\urm}{\ensuremath{\mathrm{u}}}
\newcommand{\vrm}{\ensuremath{\mathrm{v}}}
\newcommand{\wrm}{\ensuremath{\mathrm{w}}}
\newcommand{\xrm}{\ensuremath{\mathrm{x}}}
\newcommand{\yrm}{\ensuremath{\mathrm{y}}}
\newcommand{\zrm}{\ensuremath{\mathrm{z}}}

%%%capital \mathcal
\newcommand{\Acal}{\ensuremath{\mathcal{A}}}
\newcommand{\Bcal}{\ensuremath{\mathcal{B}}}
\newcommand{\Ccal}{\ensuremath{\mathcal{C}}}
\newcommand{\Dcal}{\ensuremath{\mathcal{D}}}
\newcommand{\Ecal}{\ensuremath{\mathcal{E}}}
\newcommand{\Fcal}{\ensuremath{\mathcal{F}}}
\newcommand{\Gcal}{\ensuremath{\mathcal{G}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Ical}{\ensuremath{\mathcal{I}}}
\newcommand{\Jcal}{\ensuremath{\mathcal{J}}}
\newcommand{\Kcal}{\ensuremath{\mathcal{K}}}
\newcommand{\Lcal}{\ensuremath{\mathcal{L}}}
\newcommand{\Mcal}{\ensuremath{\mathcal{M}}}
\newcommand{\Ncal}{\ensuremath{\mathcal{N}}}
\newcommand{\Ocal}{\ensuremath{\mathcal{O}}}
\newcommand{\Pcal}{\ensuremath{\mathcal{P}}}
\newcommand{\Qcal}{\ensuremath{\mathcal{Q}}}
\newcommand{\Rcal}{\ensuremath{\mathcal{R}}}
\newcommand{\Scal}{\ensuremath{\mathcal{S}}}
\newcommand{\Tcal}{\ensuremath{\mathcal{T}}}
\newcommand{\Ucal}{\ensuremath{\mathcal{U}}}
\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Wcal}{\ensuremath{\mathcal{W}}}
\newcommand{\Xcal}{\ensuremath{\mathcal{X}}}
\newcommand{\Ycal}{\ensuremath{\mathcal{Y}}}
\newcommand{\Zcal}{\ensuremath{\mathcal{Z}}}

%%%capital \mathsf
\newcommand{\Asf}{\ensuremath{\mathsf{A}}}
\newcommand{\Bsf}{\ensuremath{\mathsf{B}}}
\newcommand{\Csf}{\ensuremath{\mathsf{C}}}
\newcommand{\Dsf}{\ensuremath{\mathsf{D}}}
\newcommand{\Esf}{\ensuremath{\mathsf{E}}}
\newcommand{\Fsf}{\ensuremath{\mathsf{F}}}
\newcommand{\Gsf}{\ensuremath{\mathsf{G}}}
\newcommand{\Hsf}{\ensuremath{\mathsf{H}}}
\newcommand{\Isf}{\ensuremath{\mathsf{I}}}
\newcommand{\Jsf}{\ensuremath{\mathsf{J}}}
\newcommand{\Ksf}{\ensuremath{\mathsf{K}}}
\newcommand{\Lsf}{\ensuremath{\mathsf{L}}}
\newcommand{\Msf}{\ensuremath{\mathsf{M}}}
\newcommand{\Nsf}{\ensuremath{\mathsf{N}}}
\newcommand{\Osf}{\ensuremath{\mathsf{O}}}
\newcommand{\Psf}{\ensuremath{\mathsf{P}}}
\newcommand{\Qsf}{\ensuremath{\mathsf{Q}}}
\newcommand{\Rsf}{\ensuremath{\mathsf{R}}}
\newcommand{\Ssf}{\ensuremath{\mathsf{S}}}
\newcommand{\Tsf}{\ensuremath{\mathsf{T}}}
\newcommand{\Usf}{\ensuremath{\mathsf{U}}}
\newcommand{\Vsf}{\ensuremath{\mathsf{V}}}
\newcommand{\Wsf}{\ensuremath{\mathsf{W}}}
\newcommand{\Xsf}{\ensuremath{\mathsf{X}}}
\newcommand{\Ysf}{\ensuremath{\mathsf{Y}}}
\newcommand{\Zsf}{\ensuremath{\mathsf{Z}}}
%%%small \mathcal
\newcommand{\asf}{\ensuremath{\mathsf{a}}}
\newcommand{\bsf}{\ensuremath{\mathsf{b}}}
\newcommand{\csf}{\ensuremath{\mathsf{c}}}
\newcommand{\dsf}{\ensuremath{\mathsf{d}}}
\newcommand{\esf}{\ensuremath{\mathsf{e}}}
\newcommand{\fsf}{\ensuremath{\mathsf{f}}}
\newcommand{\gsf}{\ensuremath{\mathsf{g}}}
\newcommand{\hsf}{\ensuremath{\mathsf{h}}}
\newcommand{\isf}{\ensuremath{\mathsf{i}}}
\newcommand{\jsf}{\ensuremath{\mathsf{j}}}
\newcommand{\ksf}{\ensuremath{\mathsf{k}}}
\newcommand{\lsf}{\ensuremath{\mathsf{l}}}
\newcommand{\msf}{\ensuremath{\mathsf{m}}}
\newcommand{\nsf}{\ensuremath{\mathsf{n}}}
\newcommand{\osf}{\ensuremath{\mathsf{o}}}
\newcommand{\psf}{\ensuremath{\mathsf{p}}}
\newcommand{\qsf}{\ensuremath{\mathsf{q}}}
\newcommand{\rsf}{\ensuremath{\mathsf{r}}}
\newcommand{\ssf}{\ensuremath{\mathsf{s}}}
\newcommand{\tsf}{\ensuremath{\mathsf{t}}}
\newcommand{\usf}{\ensuremath{\mathsf{u}}}
\newcommand{\vsf}{\ensuremath{\mathsf{v}}}
\newcommand{\wsf}{\ensuremath{\mathsf{w}}}
\newcommand{\xsf}{\ensuremath{\mathsf{x}}}
\newcommand{\ysf}{\ensuremath{\mathsf{y}}}
\newcommand{\zsf}{\ensuremath{\mathsf{z}}}

%%%capital \mathbb
\newcommand{\Abb}{\ensuremath{\mathbb{A}}}
\renewcommand{\Bbb}{\ensuremath{\mathbb{B}}}
\newcommand{\Cbb}{\ensuremath{\mathbb{C}}}
\newcommand{\Dbb}{\ensuremath{\mathbb{D}}}
\newcommand{\Ebb}{\ensuremath{\mathbb{E}}}
\newcommand{\Fbb}{\ensuremath{\mathbb{F}}}
\newcommand{\Gbb}{\ensuremath{\mathbb{G}}}
\newcommand{\Hbb}{\ensuremath{\mathbb{H}}}
\newcommand{\Ibb}{\ensuremath{\mathbb{I}}}
\newcommand{\Jbb}{\ensuremath{\mathbb{J}}}
\newcommand{\Kbb}{\ensuremath{\mathbb{K}}}
\newcommand{\Lbb}{\ensuremath{\mathbb{L}}}
\newcommand{\Mbb}{\ensuremath{\mathbb{M}}}
\newcommand{\Nbb}{\ensuremath{\mathbb{N}}}
\newcommand{\Obb}{\ensuremath{\mathbb{O}}}
\newcommand{\Pbb}{\ensuremath{\mathbb{P}}}
\newcommand{\Qbb}{\ensuremath{\mathbb{Q}}}
\newcommand{\Rbb}{\ensuremath{\mathbb{R}}}
\newcommand{\Sbb}{\ensuremath{\mathbb{S}}}
\newcommand{\Tbb}{\ensuremath{\mathbb{T}}}
\newcommand{\Ubb}{\ensuremath{\mathbb{U}}}
\newcommand{\Vbb}{\ensuremath{\mathbb{V}}}
\newcommand{\Wbb}{\ensuremath{\mathbb{W}}}
\newcommand{\Xbb}{\ensuremath{\mathbb{X}}}
\newcommand{\Ybb}{\ensuremath{\mathbb{Y}}}
\newcommand{\Zbb}{\ensuremath{\mathbb{Z}}}
%%%small \mathbb
\newcommand{\abb}{\ensuremath{\mathbb{a}}}
\newcommand{\bbb}{\ensuremath{\mathbb{b}}}
\newcommand{\cbb}{\ensuremath{\mathbb{c}}}
\newcommand{\dbb}{\ensuremath{\mathbb{d}}}
\newcommand{\ebb}{\ensuremath{\mathbb{e}}}
\newcommand{\fbb}{\ensuremath{\mathbb{f}}}
\newcommand{\gbb}{\ensuremath{\mathbb{g}}}
\newcommand{\hbb}{\ensuremath{\mathbb{h}}}
\newcommand{\ibb}{\ensuremath{\mathbb{i}}}
\newcommand{\jbb}{\ensuremath{\mathbb{j}}}
\newcommand{\kbb}{\ensuremath{\mathbb{k}}}
\newcommand{\lbb}{\ensuremath{\mathbb{l}}}
\newcommand{\mbb}{\ensuremath{\mathbb{m}}}
\newcommand{\nbb}{\ensuremath{\mathbb{n}}}
\newcommand{\obb}{\ensuremath{\mathbb{o}}}
\newcommand{\pbb}{\ensuremath{\mathbb{p}}}
\newcommand{\qbb}{\ensuremath{\mathbb{q}}}
\newcommand{\rbb}{\ensuremath{\mathbb{r}}}
\newcommand{\sbb}{\ensuremath{\mathbb{s}}}
\newcommand{\tbb}{\ensuremath{\mathbb{t}}}
\newcommand{\ubb}{\ensuremath{\mathbb{u}}}
\newcommand{\vbb}{\ensuremath{\mathbb{v}}}
\newcommand{\wbb}{\ensuremath{\mathbb{w}}}
\newcommand{\xbb}{\ensuremath{\mathbb{x}}}
\newcommand{\ybb}{\ensuremath{\mathbb{y}}}
\newcommand{\zbb}{\ensuremath{\mathbb{z}}}

%%%capital \mathbbm
\newcommand{\Abbm}{\ensuremath{\mathbbm{A}}}
\newcommand{\Bbbm}{\ensuremath{\mathbbm{B}}}
\newcommand{\Cbbm}{\ensuremath{\mathbbm{C}}}
\newcommand{\Dbbm}{\ensuremath{\mathbbm{D}}}
\newcommand{\Ebbm}{\ensuremath{\mathbbm{E}}}
\newcommand{\Fbbm}{\ensuremath{\mathbbm{F}}}
\newcommand{\Gbbm}{\ensuremath{\mathbbm{G}}}
\newcommand{\Hbbm}{\ensuremath{\mathbbm{H}}}
\newcommand{\Ibbm}{\ensuremath{\mathbbm{I}}}
\newcommand{\Jbbm}{\ensuremath{\mathbbm{J}}}
\newcommand{\Kbbm}{\ensuremath{\mathbbm{K}}}
\newcommand{\Lbbm}{\ensuremath{\mathbbm{L}}}
\newcommand{\Mbbm}{\ensuremath{\mathbbm{M}}}
\newcommand{\Nbbm}{\ensuremath{\mathbbm{N}}}
\newcommand{\Obbm}{\ensuremath{\mathbbm{O}}}
\newcommand{\Pbbm}{\ensuremath{\mathbbm{P}}}
\newcommand{\Qbbm}{\ensuremath{\mathbbm{Q}}}
\newcommand{\Rbbm}{\ensuremath{\mathbbm{R}}}
\newcommand{\Sbbm}{\ensuremath{\mathbbm{S}}}
\newcommand{\Tbbm}{\ensuremath{\mathbbm{T}}}
\newcommand{\Ubbm}{\ensuremath{\mathbbm{U}}}
\newcommand{\Vbbm}{\ensuremath{\mathbbm{V}}}
\newcommand{\Wbbm}{\ensuremath{\mathbbm{W}}}
\newcommand{\Xbbm}{\ensuremath{\mathbbm{X}}}
\newcommand{\Ybbm}{\ensuremath{\mathbbm{Y}}}
\newcommand{\Zbbm}{\ensuremath{\mathbbm{Z}}}
%%%small \mathbbm
\newcommand{\abbm}{\ensuremath{\mathbbm{a}}}
\newcommand{\bbbm}{\ensuremath{\mathbbm{b}}}
\newcommand{\cbbm}{\ensuremath{\mathbbm{c}}}
\newcommand{\dbbm}{\ensuremath{\mathbbm{d}}}
\newcommand{\ebbm}{\ensuremath{\mathbbm{e}}}
\newcommand{\fbbm}{\ensuremath{\mathbbm{f}}}
\newcommand{\gbbm}{\ensuremath{\mathbbm{g}}}
\newcommand{\hbbm}{\ensuremath{\mathbbm{h}}}
\newcommand{\ibbm}{\ensuremath{\mathbbm{i}}}
\newcommand{\jbbm}{\ensuremath{\mathbbm{j}}}
\newcommand{\kbbm}{\ensuremath{\mathbbm{k}}}
\newcommand{\lbbm}{\ensuremath{\mathbbm{l}}}
\newcommand{\mbbm}{\ensuremath{\mathbbm{m}}}
\newcommand{\nbbm}{\ensuremath{\mathbbm{n}}}
\newcommand{\obbm}{\ensuremath{\mathbbm{o}}}
\newcommand{\pbbm}{\ensuremath{\mathbbm{p}}}
\newcommand{\qbbm}{\ensuremath{\mathbbm{q}}}
\newcommand{\rbbm}{\ensuremath{\mathbbm{r}}}
\newcommand{\sbbm}{\ensuremath{\mathbbm{s}}}
\newcommand{\tbbm}{\ensuremath{\mathbbm{t}}}
\newcommand{\ubbm}{\ensuremath{\mathbbm{u}}}
\newcommand{\vbbm}{\ensuremath{\mathbbm{v}}}
\newcommand{\wbbm}{\ensuremath{\mathbbm{w}}}
\newcommand{\xbbm}{\ensuremath{\mathbbm{x}}}
\newcommand{\ybbm}{\ensuremath{\mathbbm{y}}}
\newcommand{\zbbm}{\ensuremath{\mathbbm{z}}}
%%%numbers \mathbbm
\newcommand{\zerobbm}{\ensuremath{\mathbbm{0}}}
\newcommand{\onebbm}{\ensuremath{\mathbbm{1}}}
\newcommand{\twobbm}{\ensuremath{\mathbbm{2}}}
\newcommand{\fourbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\fifebbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\sixbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\sevenbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\eightbbm}{\ensuremath{\mathbbm{3}}}
\newcommand{\ninebbm}{\ensuremath{\mathbbm{3}}}


%%%capital \mathbm
\newcommand{\Abm}{\ensuremath{\bm{A}}}
\newcommand{\Bbm}{\ensuremath{\bm{B}}}
\newcommand{\Cbm}{\ensuremath{\bm{C}}}
\newcommand{\Dbm}{\ensuremath{\bm{D}}}
\newcommand{\Ebm}{\ensuremath{\bm{E}}}
\newcommand{\Fbm}{\ensuremath{\bm{F}}}
\newcommand{\Gbm}{\ensuremath{\bm{G}}}
\newcommand{\Hbm}{\ensuremath{\bm{H}}}
\newcommand{\Ibm}{\ensuremath{\bm{I}}}
\newcommand{\Jbm}{\ensuremath{\bm{J}}}
\newcommand{\Kbm}{\ensuremath{\bm{K}}}
\newcommand{\Lbm}{\ensuremath{\bm{L}}}
\newcommand{\Mbm}{\ensuremath{\bm{M}}}
\newcommand{\Nbm}{\ensuremath{\bm{N}}}
\newcommand{\Obm}{\ensuremath{\bm{O}}}
\newcommand{\Pbm}{\ensuremath{\bm{P}}}
\newcommand{\Qbm}{\ensuremath{\bm{Q}}}
\newcommand{\Rbm}{\ensuremath{\bm{R}}}
\newcommand{\Sbm}{\ensuremath{\bm{S}}}
\newcommand{\Tbm}{\ensuremath{\bm{T}}}
\newcommand{\Ubm}{\ensuremath{\bm{U}}}
\newcommand{\Vbm}{\ensuremath{\bm{V}}}
\newcommand{\Wbm}{\ensuremath{\bm{W}}}
\newcommand{\Xbm}{\ensuremath{\bm{X}}}
\newcommand{\Ybm}{\ensuremath{\bm{Y}}}
\newcommand{\Zbm}{\ensuremath{\bm{Z}}}
%%%small \mathbm
\newcommand{\abm}{\ensuremath{\bm{a}}}
\newcommand{\bbm}{\ensuremath{\bm{b}}}
\newcommand{\cbm}{\ensuremath{\bm{c}}}
\newcommand{\dbm}{\ensuremath{\bm{d}}}
\newcommand{\ebm}{\ensuremath{\bm{e}}}
\newcommand{\fbm}{\ensuremath{\bm{f}}}
\newcommand{\gbm}{\ensuremath{\bm{g}}}
\newcommand{\hbm}{\ensuremath{\bm{h}}}
\newcommand{\ibm}{\ensuremath{\bm{i}}}
\newcommand{\jbm}{\ensuremath{\bm{j}}}
\newcommand{\kbm}{\ensuremath{\bm{k}}}
\newcommand{\lbm}{\ensuremath{\bm{l}}}
\newcommand{\mbm}{\ensuremath{\bm{m}}}
\newcommand{\nbm}{\ensuremath{\bm{n}}}
\newcommand{\obm}{\ensuremath{\bm{o}}}
\newcommand{\pbm}{\ensuremath{\bm{p}}}
\newcommand{\qbm}{\ensuremath{\bm{q}}}
\newcommand{\rbm}{\ensuremath{\bm{r}}}
\newcommand{\sbm}{\ensuremath{\bm{s}}}
\newcommand{\tbm}{\ensuremath{\bm{t}}}
\newcommand{\ubm}{\ensuremath{\bm{u}}}
\newcommand{\vbm}{\ensuremath{\bm{v}}}
\newcommand{\wbm}{\ensuremath{\bm{w}}}
\newcommand{\xbm}{\ensuremath{\bm{x}}}
\newcommand{\ybm}{\ensuremath{\bm{y}}}
\newcommand{\zbm}{\ensuremath{\bm{z}}}


%%%diverse mathematical symbols and commands
\newcommand{\defas}{\mathrel{\mathop :}=} % ``defined as''-symbol
\newcommand{\asdef}{=\mathrel{\mathop :}} % ``as defined''-symbol
\newcommand{\op}[1]{\hat{\mathrm{#1}}}
\newcommand{\opsf}[1]{\hat{\mathsf{#1}}}

\newcommand{\VEV}[1]{\langle #1 \rangle}
\newcommand{\RH}{{\rm RH}}
\newcommand{\QCD}{{\rm QCD}}
\newcommand{\PQ}{{\rm PQ}}
\newcommand{\eff}{{\rm eff}}
\newcommand{\GH}{{\rm GH}}
\newcommand{\osc}{{\rm osc}}
\newcommand{\SM}{{\rm SM}}

%\newcommand{\bra}[1]{\langle #1 |}
%\newcommand{\ket}[1]{| #1 \rangle}

\renewcommand{\d}{\ensuremath{\mathrm{d}}}
%\newcommand{\ee}{\ensuremath{\mathrm{e}}}

\newcommand{\sumint}[1]{\underset{#1}{\sum\hs{-4.6mm}\int\hs{0.8mm}}}
\newcommand{\juu}{{1\hspace{-0.54ex}\mathrm{l}\hspace{-0.30ex}\mathrm{l}}} % big matrix one (three lines)
\newcommand{\hph}[1]{\hphantom{#1\;\,}}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\eps}{\varepsilon}
\newcommand{\const}{\mathrm{const}}

%%%diverse mathematical functions / operators
\newcommand{\Tr}{\ensuremath{\mathrm{Tr}}}
\newcommand{\tr}{\ensuremath{\mathrm{tr}}}
\newcommand{\sign}{\ensuremath{\mathrm{sign}}}
\newcommand{\diag}{\ensuremath{\mathrm{diag}}}
\newcommand{\Vol}{\ensuremath{\mathrm{Vol}}}
\newcommand{\Ker}{\ensuremath{\mathrm{Ker}}}

%%%diverse physical energy units
\newcommand{\mueV}{\ensuremath{\, \mu\mathrm{eV}}}
\newcommand{\meV}{\ensuremath{\, \mathrm{meV}}}
\newcommand{\eV}{\ensuremath{\, \mathrm{eV}}}
\newcommand{\keV}{\ensuremath{\, \mathrm{keV}}}
\newcommand{\MeV}{\ensuremath{\, \mathrm{MeV}}}
\newcommand{\GeV}{\ensuremath{\, \mathrm{GeV}}}
\newcommand{\TeV}{\ensuremath{\, \mathrm{TeV}}}
\newcommand{\PeV}{\ensuremath{\, \mathrm{PeV}}}

\newcommand{\cm}{\ensuremath{\, \mathrm{cm}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%MISCELLANEOUS
\newcommand{\ub}[3]{\underbrace{#1}_{\phantom{#3}\,#2\,#3}}
\newcommand{\ob}[3]{\overbrace{#1}^{\phantom{#3}\,#2\,#3}}
%\newcommand{\ol}{\overline}
\renewcommand{\u}{\underline}
\newcommand{\os}{\overset}
\newcommand{\us}{\underset}

\newcommand{\cds}{\,\cdot\,}

\newcommand{\eg}{eg.}
\newcommand{\ie}{i.e.}
\newcommand{\etal}{et al.}
\newcommand{\hc}{{\rm H.c.}}
\newcommand{\rhs}{r.h.s.}
\newcommand{\lhs}{l.h.s.}
\newcommand{\wrt}{w.r.t.}
\newcommand{\cf}{cf.}

\newcommand{\jd}[1]{\textcolor{orange}{Johannes: #1}}
\newcommand{\ek}[1]{\textcolor{blue}{Emi: #1}}
\newcommand{\me}[1]{\textcolor{red}{Manu: #1}}


\setlength{\parskip}\smallskipamount
%\linespread{1.2}

\setlength{\footnotesep}{3.5mm}

%\def\theequation{\thesection.\arabic{equation}}

\settimeformat{ampmtime}

\usepackage{float}

%\numberwithin{equation}{section}

%\binoppenalty=\maxdimen
%\relpenalty=\maxdimen

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\FK}[1]{\color{orange}{#1\;}\color{black}}
\newcommand{\BC}[1]{\color{red}{#1\;}\color{black}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% *****************************************************************
% ********************** END HEADER *************************
% *****************************************************************

